Deriving Neural Architectures from Sequence and Graph Kernels

The design of neural architectures for structured objects is typically guided by experimental insights rather than a formal process. In this work, we appeal to kernels over combinatorial structures, such as sequences and graphs, to derive appropriate neural operations. We introduce a class of deep recurrent neural operations and formally characterize their associated kernel spaces. Our recurrent modules compare the input to virtual reference objects (cf. filters in CNN) via the kernels. Similar to traditional neural operations, these reference objects are parameterized and directly optimized in end-to-end training. We empirically evaluate the proposed class of neural architectures on standard applications such as language modeling and molecular graph regression, achieving state-of-the-art results across these applications.

==> discussion.tex <==
\section{Discussion}

We proposed a class of deep recurrent neural architectures and formally characterized its underlying computation using kernels.
Our derivation provides a mechanism for designing networks -- by linking kernel and neural operations, we have a ``template'' for deriving new families of neural architectures, for different types of combinatorial structures.

Interestingly, many recent work has reached similar empirical observations when exploring different RNN variants. \citet{greff2015lstm} found that simplifying LSTMs, for instance, by removing the input gate or coupling it with the forget gate does not significantly change the performance.
However, the forget gate (corresponding to the decay factor $\lambda$ in our notation) is crucial for performance.
This is consistent with our theoretical analysis and the empirical results in Figure~\ref{fig:lm-ana}.
Moreover, \citet{BalduzziG16} and \citet{ran17} both suggest that a linear additive state computation suffices to provide competitive performance compared to LSTMs:
\footnote{\citet{BalduzziG16} also includes the previous token , i.e. $\W \x_t + \W' \x_{t-1}$, which doesn't affect the discussion here.}
\begin{align*}
 \mbf{c}[t] &= \lambda_f \odot \mbf{c}_1[t-1] + \lambda_i\odot \left(\W \x_t\right)\\
 \mbf{h}[t] &= \sigma(\mbf{c}[t])
\end{align*}
This variant is indeed an instance of the kernel-derived neural class presented in this work (with $n=1$ and adaptive gating).
We hope our theoretical view of our novel recurrent operations can be helpful for future model exploration.
%Indeed, by tuning the hyper-parameters associated with the networks (such as depth $L$ and feature width $n$), we were able to achieve state-of-the-art performance across various tasks.


